GraphBLAST: A High-Performance Linear Algebra-based Graph Framework on the GPU

High-performance implementations of graph algorithms are challenging to implement on new parallel hardware such as GPUs because of three challenges: (1) the difficulty of coming up with graph building blocks, (2) load imbalance on parallel hardware, and (3) graph problems having low arithmetic intensity. To address some of these challenges, GraphBLAS is an innovative, on-going effort by the graph analytics community to propose building blocks based on sparse linear algebra, which will allow graph algorithms to be expressed in a performant, succinct, composable and portable manner. In this paper, we examine the performance challenges of a linear-algebra-based approach to building graph frameworks and describe new design principles for overcoming these bottlenecks. Among the new design principles is exploiting input sparsity, which allows users to write graph algorithms without specifying push and pull direction. Exploiting output sparsity allows users to tell the backend which values of the output in a single vectorized computation they do not want computed. Load-balancing is an important feature for balancing work amongst parallel workers. We describe the important load-balancing features for handling graphs with different characteristics. The design principles described in this paper have been implemented in "GraphBLAST", the first high-performance linear algebra-based graph framework on NVIDIA GPUs that is open-source. The results show that on a single GPU, GraphBLAST has on average at least an order of magnitude speedup over previous GraphBLAS implementations SuiteSparse and GBTL, comparable performance to the fastest GPU hardwired primitives and shared-memory graph frameworks Ligra and Gunrock, and better performance than any other GPU graph framework, while offering a simpler and more concise programming model.

==> alg/rowcolbased.tex <==
\bcolorbox
\begin{minipage}[]{\textwidth}
\begin{minipage}[]{0.48\textwidth}
  \renewcommand{\algorithmicrequire}{\textbf{Input:}}
  \renewcommand{\algorithmicensure}{\textbf{Output:}}
  \begin{algorithmic}[1]
  	\Require{Sparse Matrix $\mA$, Dense Vector $\mathbf{x}$}
  	\Ensure{Dense Vector $\mathbf{y}$}
    \Procedure{SpMV}{$\mA, \mathbf{x}, \mathbf{y}$}
    \For{$i$ = 0 to $\mA$.nrows $-1$}
	    \State{}$\mathbf{y}(i) \leftarrow$ $\mA(i,:) \mathbf{x}$
    \EndFor{}
    \EndProcedure{}
  \end{algorithmic}
  \captionof{algorithm}{SpMV only exploits input matrix sparsity $\mA(i,:)$.\label{alg:rowbased}}
\end{minipage}
\hfill
\begin{minipage}[]{0.48\textwidth}
	\renewcommand{\algorithmicrequire}{\textbf{Input:}}
	\renewcommand{\algorithmicensure}{\textbf{Output:}}
	\begin{algorithmic}[1]
		\Require{Sparse Matrix $\mA$, Sparse Vector $\mathbf{x}$}
		\Ensure{Sparse Vector $\mathbf{y}$}
		\Procedure{SpMSpV}{$\mA, \mathbf{x}, \mathbf{y}$}
		\For{$i$ s.t. $\mathbf{x}(i) \neq 0$}
		\State{}$\mathbf{y} \leftarrow$ $\mA(:,i) \mathbf{x}(i)$
		\EndFor{}
		\EndProcedure{}
	\end{algorithmic}
	\captionof{algorithm}{SpMSpV exploits both input vector sparsity ($i \text{ s.t. } \mathbf{x}(i) \neq 0$) and input matrix sparsity $\mA(:,i)$.\label{alg:colbased}}
\end{minipage}
\end{minipage}
\ecolorbox

==> fig/perf.tex <==
\begin{figure}[t]
        \begin{subfigure}[t]{\textwidth}
                \centering
                \includegraphics[width=\textwidth]{fig/mteps}
                \centering
                \caption{Performance (MTEPS) [higher is better]\label{fig:mteps}}
        \end{subfigure}
        \begin{subfigure}[t]{\textwidth}
                \centering
                \includegraphics[width=\textwidth]{fig/elapsed}
                \centering
                \caption{Runtime (ms) [lower is better]\label{fig:elapsed}}
        \end{subfigure}
        \caption[Performance comparison for GraphBLAST\@.]{Performance in MTEPS and milliseconds for GraphBLAST vs.\ four other graph processing libraries and hardwired algorithms on different graph inputs. Data is from Table~\ref{tab:exp_largetable}.\John{So I don't like these graphs. They are designed with the idea that it is meaningful to compare runtime or MTEPS across primitives. I don't think it is. I don't think anyone cares that in general PR has slightly better MTEPS than SSSP\@. As a result, each graph has very little dynamic range between highest and lowest, so most of the vertical space is wasted.

        Instead, I think you want to normalize each graph to a baseline (perhaps SuiteSparse?). Then plot speedup. Each graph can have a different y axis.

        As well, I \emph{believe} that a dot plot is better than a bar plot, because all the ink you're using in the bars delivers no value.  \url{https://www.perceptualedge.com/articles/b-eye/dot_plots.pdf   http://www.maartenlambrechts.com/2015/05/03/to-the-point-7-reasons-you-should-use-dot-graphs.html}}\label{fig:perf-journal}}
\end{figure}


==> table/cora.tex <==
\begin{table}[t]
	\centering
	\begin{tabular}{ccc|cc|cc|cc}
		\toprule
		 & & & \multicolumn{2}{c|}{Cora} & \multicolumn{2}{c|}{Citeseer} & \multicolumn{2}{c}{Wiki} \\
		 & Type & Info & Acc & Avg Entr & Acc & Avg Entr & Acc & Avg Entr \\ \midrule
		K-means & U & Content & 0.4922 & 1.7979 & 0.5401 & 1.7543 & 0.4172 & 2.1241 \\ 
		Spectral & U & Structure & 0.3672 & 2.4408 & 0.2389 & 2.4451 & 0.2204 & 3.0891 \\ 
		Big-Clam [1] & U & Structure & 0.2718 & 2.6287 & 0.2500 & 2.4614 & 0.1563 & 3.3690 \\
		GraphEncoder [2] & U & Structure & 0.3249 & 2.4598 & 0.2252 & 2.4785 & 0.2067 & 3.2770 \\
		DeepWalk [3] & U & Structure & 0.4840 & 1.8140 & 0.3365 & 2.3079 & 0.3846 & 2.4514 \\
		DNGR [4] & U & Structure & 0.4191 & 1.8816 & 0.3259 & 2.1675 & 0.3758 & 2.2605 \\ \midrule
		This work & U & Structure & 0.2740 & 1.8397 & 0.2268 & 1.5866 & 0.3260 & 2.8786 \\ \midrule
		Circles [5] & U & Both & 0.6067 & 1.5563 & 0.5716 & 1.7751 & 0.4241 & 2.0038 \\
		RTM [6] & U & Both & 0.4396 & 2.0208 & 0.4509 & 1.9154 & 0.4364 & 2.0458 \\
		RMSC [7] & U & Both & 0.4066 & 2.1097 & 0.2950 & 2.2770 & 0.4150 & 2.2201 \\
		TADW [8] & SS & Both & 0.5603 & 1.6052 & 0.4548 & 1.9160 & 0.3976 & 2.9080 \\
		VGAE [9] & SS & Both & 0.5020 & 1.7541 & 0.4670 & 1.8630 & 0.4509 & 1.8510 \\
		\bottomrule
	\end{tabular}
\end{table}

\begin{table}[t]
	\centering
	\begin{tabular}{c|c|cccccc}
		\toprule
		& Information & Accuracy & F-score & Precision & Recall & Avg. & ARI \\
		& & & & & & Entropy & \\ \midrule
		K-means & Content & & 0.2628 & 0.2108 & 0.2592 & 2.1241 & 0.1507 \\ 
		Spectral & Structure & 0.2204 & 0.1757 & 0.1055 & 0.5243 & 3.0891 & 0.0146 \\ 
		Big-Clam [1] & Structure & 0.1563 & 0.1638 & 0.0946 & 0.6117 & 3.3690 & 0.0070 \\
		GraphEncoder [2] & Structure & 0.2067 & 0.1717 & 0.1006 & 0.5936 & 3.2770 & 0.0049 \\
		DeepWalk [3] & Structure & 0.3846 & 0.2574 & 0.2418 & 0.2779 & 2.4514 & 0.1703 \\
		DNGR [4] & Structure & 0.3758 & 0.2538 & 0.2773 & 0.2353 & 2.2605 & 0.1797 \\ \midrule
		This work & Structure & 0.3260 & 0.2069 & 0.2740 & 0.1662 & 2.8786 & 0.1434 \\ \midrule
		Circles [5] & Both & 0.4241 & 0.3035 & 0.3662 & 0.2592 & 2.0038 & 0.2420 \\
		RTM [6] & Both & 0.4364 & 0.2481 & 0.1920 & 0.3539 & 2.0458 & 0.1384 \\
		RMSC [7] & Both & 0.4150 & 0.2344 & 0.1672 & 0.3975 & 2.2201 & 0.1116 \\
		TADW [8] & Both & 0.3976 & 0.2068 & 0.1203 & 0.7538 & 2.9080 & 0.0454 \\
		VGAE [9] & Both & 0.4509 & 0.4676 & 0.3687 & 0.2957 & 1.8510 & 0.2634 \\
		MGAE [10] & Both & 0.5293 & 0.5104 & 0.5178 & 0.3671 & 1.6676 & 0.3787 \\	\bottomrule
	\end{tabular}
\end{table}

==> table/generalize.tex <==
\begin{table}[t]
	\centering
\begin{tabular}{cccc}
	\toprule
	BFS Optimization & & GraphBLAST Feature & Section \\ \midrule
	Change of direction & $\rightarrow$ & Generalized direction-optimization & \\
	Structure only & $\rightarrow$ & Boolean semiring & Section~\ref{sec:diropt}:\\
	Early exit  & $\rightarrow$ & Boolean semiring & Direction-optimization \\
	Operand reuse & $\rightarrow$ & Avoid sparse-to-dense conversion  & \\ \midrule
	Fused mask  & $\rightarrow$ & Generalized masking & Section~\ref{sec:masking}: Masking \\ \midrule
	Per vertex & $\rightarrow$ & Static mapping & Section~\ref{sec:loadbalancing}: \\
	Per edge & $\rightarrow$ & Dynamic mapping (merge-based) & Load-balancing \\ \bottomrule
\end{tabular}
	\caption{Generalizeability of design features.\label{tab:generalize}}
\end{table}
